Intelligent Traffic Monitoring with Hybrid AI

Challenges in Intelligent Traffic Monitoring (ITMo) are exacerbated by the large quantity and modalities of data and the need for the utilization of state-of-the-art (SOTA) reasoners. We formulate the problem of ITMo and introduce HANS, a neuro-symbolic architecture for multi-modal context understanding, and its application to ITMo. HANS utilizes knowledge graph technology to serve as a backbone for SOTA reasoning in the traffic domain. Through case studies, we show how HANS addresses the challenges associated with traffic monitoring while being able to integrate with a wide range of reasoning methods

==> Sections-demo/Ackno.tex <==
We would like to thank Emil Schreiber and Florian Richter from Bosch Security Systems for the constructive comments to the present contribution and the continuous support to the project. 

==> Sections/Abstract.tex <==
\begin{abstract}
    Bridging the gap in state-of-the-art reasoning and challenges in traffic domain is exacerbated by the large quantity
    of data which needs to be processed.
    In this work, we present TrafficKG, a knowledge resource facilitating the integration of large quantities of multi-modal data with SOTA reasoning for traffic data analysis. Our results show that ...
\end{abstract}

==> Sections/Conclusion.tex <==
TBD

==> Sections/Experiments.tex <==
\subsection{Setup and Data Details}
Details of the video data we will use to generate scene part of TrafficKG

\subsection{TrafficKG Stats}
Stats associated to TrafficKG and its three main parts.

\subsection{Baseline Traffic Congestion Results}
Baseline rule-based traffic congestion results

\subsection{Unsupervised Scene Similarity}
Results on scene similarity using different algorithms
\subsubsection{Using Graph Structure}
results from Stardogs node similarity
\subsubsection{Using Lexical Similarity}
results from lexical similarity from Stardog simple methods
\subsubsection{Using Semantic Similarity}
results from fine-tuning a language model on background knowledge


==> Sections/Introduction.tex <==
%%%%%%%%%%%%%%%%%%%%% Why Traffic Monitoring is important
Traffic monitoring and management is one of the main challenges in today's smart cities with thousands of travels per day\cite{das2019smart}.
With the advent of autonomous cars, cheap sensory data from cities, and artificial intelligence, the opportunities for smart monitoring and interfering in the traffic flow is more achievable \cite{chowdhury2021towards}.


\proska{more details here on how each helps} 


%%%%%%%%%%%%%%%%%%%%% Why work on Traffic monitoring
\proska{need more previous work}



%%%%%%%%%%%%%%%%%%%%% What is lacking in the previous work
We identify four main challenges associated with task of reasoning with traffic data.
First, traffic data inherently involves reasoning over large quantities of data. 
This data can include transient information such as videos from traffic cameras, acoustic sensing~\cite{lancelle2016distributed}, and even weather report~\cite{yu2017deep}. 
In addition to sensory data, any system reasoning over traffic data must have background knowledge on mechanics of traffic flow and implicit assumptions humans would make in their interactions formally known as commonsense knowledge\cite{ilievski2020consolidating}.
Second, any reasoning system on traffic data must have a flexible design for future development.
Third, it must have simple integration with SOTA reasoners, both symbolic and neural.
Finally, It must be able to handle the noisy associated with sensory data outputs.


%%%%%%%%%%%%%%%%%%%%% Start talking about our contributions
Our solution:
Hybrid Reasoning for Traffic Data Analysis
Use Knowledge Graph technology to integrate large quantities of data
Semantic model provides coherent and consistent data representation and management
Easy gradual development
Flexible and simple query mechanism (SPARQL)
Easy integration with available KGs to provide prior knowledge
Commonsense knowledge
Factual knowledge
Well studied reasoning pipeline in research literature: 
Rule-based reasoning (baseline)
Neuro-symbolic and multi-modal reasoning



%%%%%%%%%%%%%%%%% First contribution: Ontology


%%%%%%%%%%%%%%%%% Second contribution: Knowledge consolidation


%%%%%%%%%%%%%%%%% Third contribution: Hybrid Reasoning

==> Sections/ProblemFormulation.tex <==
In traffic data monitoring, we are given large quantity of data in different modalities. 
For example, we have access to raw video footage of traffic cameras in a region. 
For each camera we may also have associated meta-data such as coordinates, frame-rate, or description of the traffic entity the camera is looking e.g intersection or highway.
We also have access to public knowledge such as map of the region, e.g. \OSM ~\cite{OpenStreetMap}, the weather information of the region, e.g. OpenWeatherMap
\footnote{\hyperlink{https://openweathermap.org/}{https://openweathermap.org/}}
, or historical traffic information, e.g. SigAlert~\cite{walton2011livelayer}.

In addition to such regional transient knowledge, we also have access to general knowledge associated with traffic data.
This general knowledge includes factual knowledge, such as what each traffic light color means, and \CSn knowledge such as cars don't fly (at least for now). 
Here \CSn knowledge refers to set of assumptions and beliefs that are acceptable by people without need for debate~\cite{sap2019atomic,ilievski2020consolidating}.
It can be of temporal nature, e.g. pushing gas pedal causes acceleration, spacial, e.g. two cars cannot be in same location, or even cultural, e.g. Pittsburgh left.

The goal in traffic data monitoring is then to use this data, for automatic decision making and perform reasoning to answer queries such as \QT{Is there any traffic congestion?} or \QT{Are there any accidents?}.
There are four main challenges associated with traffic data monitoring. First, the multi-modal nature of data and its inordinate size complicates task of using the data. 
Second, any system for traffic data monitoring must be flexible enough for future development. 
Third, it must have easy integration with state-of-the-art(SOTA) reasoners. 
Finally, it must be able to handle sheer amount of noise in the data sources \proska{needs citation}. 

In this work, to showcase TrafficKG, we simply focus on a subset of input data. 
We assume we have access to real-time video feeds from traffic camera, the meta-data associated with each camera, and general knowledge associated with traffic data.
% In this section we are going to discuss the details of the available video data and the type of annotations we expect to have access to using off-the-shelf video processing tools (e.g. detected objects, speed, trajectory).

% Next, we are going to discuss a couple of scenarios in which a reasoner would help the urban decision making process. 

% Finally we will discuss the challenges of such problem: 1.Large quantity of data, 2.Flexible system for future development, 3.Integration with SOTA reasoners, and 4.Noisy Detection Outputs.


==> Sections/TMO.tex <==
To facilitate the management of multi-modal traffic data, future development and simple integration with SOTA reasoners, we propose Traffic Monitoring Ontology~(TMO). 
TMO~(figure \ref{fig:tmo}) builds on top of SSN~\cite{haller2019modular} and Scene Ontology \proska{needs citation} with expanded traffic domain information.

TMO, uses knowledge graph technology to store the parsed information

\begin{figure}
    \centering
    \includegraphics[width=.7\columnwidth]{Assets/TMO.png}
    \caption{Traffic Monitoring Ontology}
    \label{fig:tmo}
\end{figure}

==> Sections/TrafficKG.tex <==
This section summarizes the available resources for knowledge related to traffic. The goal here is to consolidate this information that can be used as backbone knowledge for any type of reasoning on the traffic scenes. 

Generally speaking, we have grouped the resources into 3 groups: \QT{Scene Knowledge}~(\ref{subsec:sceneknowledge}) that consist of the information obtained from the visual analysis of traffic camera feeds and post processed data including the entities in the scene or topology of the street, \QT{Factual Knowledge}~(\ref{subsec:factualknowledge}) that includes factual information about the type of entities we may need to reason about and their mechanics, including traffic light's colors and their meanings, or cars features, etc., and finally the \QT{Commonsense Knowledge}~(\ref{subsec:csknowledge}) that allows the reasoner to infer the intent and purpose of each entities action and limitations given the context (e.g. Cars on a car carrier trailer cannot move independently).

For each resource, we first briefly introduce the resource. We then discuss the type of traffic-related information we can potentially obtain from it. Finally, we illustrate the use-case of the resource with an example from it and discuss the type of reasoning one can do using the information.  

\subsection{Scene Knowledge}
\label{subsec:sceneknowledge}
Scene knowledge contains the type of knowledge that can be obtained from analyzing the traffic camera feeds.
Using off-the-shelf image processing techniques we are also able to extract information such as the entities that are present in the scene, or the topology of the street. 
This type of information coupled with background knowledge on traffic and transportation can be used by the reasoning system to detect different traffic phenomena such as congestion.
The diagram below illustrates the type of information we expect to get from the video feed. 
In this diagram, the static and dynamic terminology respectively refer to the static elements in the scene such as roads and dynamic elements are the moving ones such as cars. 
Using only the scene knowledge although the reasoner can learn that there is car in it, however it does not know what a car is a what is capable of. 
Hence, In order to use this scene information, we need to provide the reasoner with additional information about each entity in the scene that will be covered by factual and commonsense knowledge.

\subsection{Factual Knowledge}
\label{subsec:factualknowledge}
This group contains factual knowledge of the entities, topics, and objects related to traffic. 
All these resources have a strong community of human annotators that constantly update, add, and maintain the knowledge on them.
The main goal of having such knowledge is to provide basic information on the general mechanics of the entities and their main features such as types of road, and simple topological information such as number lanes or road type information for the reasoner.

\subsection{Commonsense Knowledge}
\label{subsec:csknowledge}
Common sense knowledge allows the reasoner based on TrafficKG to have the ability to understand the possible intent, purpose and outcome of the actions performed by the entities. Gathering knowledge related to this group is most probably the most difficult part of creating TrafficKG as by definition Commonsense Knowledge is rarely written down by humans. In addition, the Commonsense knowledge is mostly being considered as the "reading between the lines" ability of humans which makes it more difficult to formulate. 

In recent years, there have been many efforts to gather such knowledge using different automatic and hand annotated methods. The following resources are among the well-stablished resources available online.


\section{Hybrid Reasoning}

\subsection{Baseline Reasoning}


\subsection{Bridging the Modal Inconsistency with Lexicalization}
\begin{itemize}
\item Number of detected objects: “There are 8 object(s) in the scene.”
\item Object composition: “From the object(s), 3 are car, 2 are person, 1 is a truck, and 2 are unknown. ”
\item Speed of objects: “The first car is moving with the average speed of 6.0 m/s. The second car is moving with the average speed of 1.76 m/s. The third car is moving with the average speed of 8.0 m/s. The first person is moving with the average speed of 5.0 m/s. The first truck is moving with the average speed of 6.9 m/s.”
\item Location of objects: “In lane 6 we see first car, second car, third car, first person, and first truck.”

\end{itemize}
\subsection{Injecting the Background Knowledge into Reasoner}
Details on lexicalizing the background knowledge and use them to fine-tune the language model.

\subsection{Unsupervised Scene Similarity}
introduction to the unsupervised scene similarity as an intermediate task to evaluate the system without the use of ground truth.

